LMDepth: Lightweight Mamba-based Monocular Depth Estimation for Real-World Deployment

Monocular depth estimation provides an additional depth dimension to RGB images, making it widely applicable in various fields such as virtual reality, autonomous driving and robotic navigation. However, existing depth estimation algorithms often struggle to effectively balance performance and computational efficiency, which poses challenges for deployment on resource-constrained devices. To address this, we propose LMDepth, a lightweight Mamba-based monocular depth estimation network, designed to reconstruct high-precision depth information while maintaining low computational overhead. Specifically, we propose a modified pyramid spatial pooling module that serves as a multi-scale feature aggregator and context extractor, ensuring global spatial information for accurate depth estimation. Moreover, we integrate multiple depth Mamba blocks into the decoder. Designed with linear computations, the Mamba Blocks enable LMDepth to efficiently decode depth information from global features, providing a lightweight alternative to Transformer-based architectures that depend on complex attention mechanisms. Extensive experiments on the NYUDv2 and KITTI datasets demonstrate the effectiveness of our proposed LMDepth. Compared to previous lightweight depth estimation methods, LMDepth achieves higher performance with fewer parameters and lower computational complexity (measured by GFLOPs). We further deploy LMDepth on an embedded platform with INT8 quantization, validating its practicality for real-world edge applications.

==> table/table1.tex <==
\begin{table*}[t]
    \centering
    %
    \caption{Comparison of performances on the KITTI dataset. The reported numbers are from the corresponding original papers. Measurements are made for the depth range from $0m$ to $80m$. Best / Second best results are marked \textbf{bold} / \underline{underlined}. E-B5 are short for EfficientNet-B5~\cite{tan2019efficientnet}. \dag and \ddag represent the models are pre-trained by ImageNet-22K and auxiliary depth estimation dataset, respectively.}
    %
    \label{tab::results-kitti-val}
    \scalebox{0.7}{%
        \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
            \hline
            Method & Ref & Backbone & ~~~\textbf{$\delta_1$}$\uparrow$~~~ & ~~~\textbf{$\delta_2$}$\uparrow$~~~ & ~~~\textbf{$\delta_3$}$\uparrow$~~~ & ~REL~$\downarrow$~ & Sq-rel~$\downarrow$ & RMS~$\downarrow$ & RMS log~$\downarrow$ \\
            \hline
            % Saxena~\etal~\cite{saxena2005learning} & - & 0.601 & 0.820  & 0.926 & 0.280   & 3.012  & 8.734 & 0.361    \\
            % Eigen~\etal~\cite{eigen2014depth} & Convolutions & 0.702 & 0.898 & 0.967 & 0.203   & 1.548  & 6.307 & 0.282    \\
            % Liu~\etal~\cite{liu2015learning} & Convolutions & 0.680 & 0.898 & 0.967 & 0.201   & 1.584  & 6.471 & 0.273    \\
            Godard~\etal~\cite{godard2017unsupervised}& CVPR 2017 & ResNet-50 & 0.861 & 0.949 & 0.976 & 0.114   & 0.898  & 4.935 & 0.206 \\
            Johnston~\etal~\cite{johnston2020self}& CVPR 2020 & ResNet-101 & 0.889 & 0.962 & 0.982 & 0.106 & 0.861 & 4.699 & 0.185 \\
            Gan~\etal~\cite{gan2018monocular}& ECCV 2018 & ResNet-101 & 0.890 & 0.964 & 0.985 & 0.098   & 0.666  & 3.933 & 0.173 \\
            % PLADE-Net~\cite{gonzalez2021plade} & FAL-Net & 0.900 & 0.967 & 0.985 & 0.089 & 0.590 & 4.008 & 0.172\\
            DORN~\etal~\cite{fu2018dorn}& CVPR 2018 & ResNet-101 & 0.932 & 0.984 & 0.994 & 0.072   & 0.307  & 2.727 & 0.120\\
            Yin~\etal~\cite{yin2019enforcing}& ICCV 2019 & ResNext-101 & 0.938 & 0.990  & \underline{0.998} & 0.072 & -- & 3.258 & 0.117 \\
            PGA-Net~\cite{xu2020probabilistic}& TPAMI 2020 & ResNet-50 & 0.952 & 0.992 & \underline{0.998} & 0.063 & 0.267 & 2.634 & 0.101 \\
            BTS~\cite{lee2019bts}& Arxiv 2019 & DenseNet-161& 0.956 & 0.993 & \underline{0.998} & 0.059   & 0.245  & 2.756 & 0.096 \\
            TransDepth~\cite{yang2021transdepth}& ICCV 2021 & ResNet-50+ViT-B\dag & 0.956 & 0.994 & \textbf{0.999} & 0.064 & 0.252  & 2.755 & 0.098 \\
            DPT~\cite{ranftl2021dpt} & ICCV 2021 &ResNet-50+ViT-B\ddag & 0.959 & 0.995 & \textbf{0.999} & 0.062 & --& 2.573 & 0.092 \\
            AdaBins~\cite{bhat2021adabins} & CVPR 2021 &E-B5+mini-ViT & 0.964 & 0.995 & \textbf{0.999} & 0.058  & 0.190  & 2.360 & 0.088\\
            \hline
            \multirow{6}{*}{\textbf{BinsFormer}} & \multirow{6}{*}{\textbf{Ours}}
             & ResNet-18  & 0.954 & 0.994 & \textbf{0.999} & 0.065 & 0.230 & 2.574 & 0.099 \\
            \hline
        \end{tabular}
    }
\end{table*}
